The Theory of Call-by-Value Solvability (long version)

The denotational semantics of the untyped lambda-calculus is a well developed field built around the concept of solvable terms, which are elegantly characterized in many different ways. In particular, unsolvable terms provide a consistent notion of meaningless term. The semantics of the untyped call-by-value lambda-calculus (CbV) is instead still in its infancy, because of some inherent difficulties but also because CbV solvable terms are less studied and understood than in call-by-name. On the one hand, we show that a carefully crafted presentation of CbV allows us to recover many of the properties that solvability has in call-by-name, in particular qualitative and quantitative characterizations via multi types. On the other hand, we stress that, in CbV, solvability plays a different role: identifying unsolvable terms as meaningless induces an inconsistent theory.

==> 05-Genericity.tex <==
% !TEX root = main.tex
\section{Genericity and the Consistency of the Smallest Sensible Theory $\Hv$}
\label{sect:genericity}
Here we prove the \emph{genericity (lemma)} of \cbv \emph{un}solvability, which implies the consistency of the extension $\Hv$ of $=_{\vsub}$ that equates all unsolvable \VSC terms. Genericity states that if $\tm$ has an unsolvable sub-term $\tmtwo$ and it normalizes, then $\tmtwo$ is useless for normalizing, and so $\tm$ normalizes even if one replaces $\tmtwo$ with an arbitrary term. Genericity can also be taken as an alternative definition of \cbn solvability, as noted by Garc\'ia-P\'erez and Nogueira \cite{DBLP:journals/corr/Garcia-PerezN16}. 
%by Garc\'ia-P\'erez and Nogueira \cite{DBLP:journals/corr/Garcia-PerezN16}. 

We adapt a simple direct proof for \cbn by Takahashi \cite{DBLP:conf/birthday/Takahashi94}, who obtains genericity---that is usually formulated via contexts, see Barendregt \cite[Prop.~14.3.24]{Barendregt84}---as a corollary of a formulation via substitutions. We also replace conversion with~reduction. Alternative proofs of both genericity and consistency of $\Hv$ can be obtained by proving the axioms by Kennaway et al. \cite{DBLP:journals/jflp/KennawayOV99}, as discussed at the end of the section.

\mysubparagraph{A Key Point} Takahashi's proof uses a key property of the reduction characterizing solvability---head reduction $\toh$ in her case (\cbn)---namely its \emph{stability under substitutions}: if $\tm \toh^{*} \tmtwo$ then $\tm\isub\var\tmthree \toh^{*} \tmtwo\isub\var\tmthree$ for every $\var$ and $\tmthree$. As we have seen in \Cref{ssect:irrelevance}, such a property does not hold for solving reduction $\tosolv$ in the \VSC, as it fails for $\toevar$ steps.
In our setting, the solution is easy: just consider $\tosolvnvar$ rather than $\tosolv$ for which stability by substitutions hold.


Takahashi \cite{DBLP:conf/birthday/Takahashi94} does not stress  the relevance of stability by substitution, but she does stress one of its consequences, given by the next lemma. 

%\begin{proposition}[Irrelevance of $\toevar$]
%	\label{prop:irrelevance}
%	\NoteProof{propappendix:irrelevance}
%	\hfill
%	\begin{enumerate}
%		\item\label{p:irrelevance-postponement} \emph{Postponement}: if $\deriv \colon \tm \, \tovsub^*\, \tmtwo$ then there is $\derivp \colon \tm \tovsubnvar^* \!\cdot \toevar^* \, \tmtwo$ with $\sizem\derivp = \sizem \deriv$;
%		\item\label{p:irrelevance-postponement-solv} \red{\emph{Postponement}: if $\deriv \colon \tm \, \tosolv^*\, \tmtwo$ then there is $\derivp \colon \tm \tosolvnvar^* \!\cdot \toevarsolv^* \, \tmtwo$ with $\sizem\derivp = \sizem \deriv$};
%
%%		\item\emph{Strong normalization}: $\toevar$ is strongly normalizing.
%		\item\label{p:irrelevance-termination} \emph{Termination}: a term is weakly (\resp strongly) normalizing for $\tovsub$ if and only if so is it for $\tom \!\cup \toeabs$. \red{Moreover, $\tosolv$ terminates if and only if $\tosolvnvar$ terminates.}
%	\end{enumerate}
%\end{proposition}

%It is easily seen that a term is $\tosolvnvar$ normal if and only if it has the following shape:
%\begin{center}
%		$\textsc{Lax solvable fireballs} \qquad \lsolvnf \grameq  \itm \mid \la{\var}\lsolvnf \mid \lsolvnf \esub{\var}{\itm}$
%\end{center}
\begin{lemma}[Stability of solvability under removal]
\label{l:stability-solv-subs} % \Cref{l:stability-solv-subs}.\ref{p:stability-solv-subs-two}
If there exists $\tmtwo$ such that $\tm\isub\var\tmtwo$ is solvable then $\tm$ is solvable.
\end{lemma}
The rest of Takahashi's proof then smoothly adapts. Actually, her proof also relies on the normalization theorem for head reduction, even if she does not point it out. Similarly, our proof uses the normalization property for $\tosolvnvar$ (\Cref{prop:properties-solving}.\ref{p:properties-solving-normalization-bis}).

The statement of the genericity property is about reductions to full normal form, which here are exactly \emph{full fireballs}. The first point of the next theorem is the crucial statement, the second---which is what is usually considered the genericity property---is an immediate consequence.

\begin{theorem}[Genericity]
\label{thm:genericity}
\NoteProof{thmappendix:genericity}
Let $\tm$ be an unsolvable term and $\tmtwo$ a full normal form.
\begin{enumerate}
\item \label{p:genericity-as-subs}
\emph{Genericity as substitution}:
if $\tmthree \isub\var\tm \tovsub^{*} \tmtwo$ then $\tmthree \isub\var\tmfour \tovsub^{*} \tmtwo$ for every term $\tmfour$.

\item \emph{Genericity as context}:
if $\ctxp\tm \tovsub^{*} \tmtwo$ then $\ctxp\tmthree \tovsub^{*} \tmtwo$ for every term $\tmthree$.
\end{enumerate}
\end{theorem}

\mybigsubparagraph{The Smallest Sensible Theory $\Hv$} By a standard easy construction (Barendregt \cite[pp. 412-414]{Barendregt84}), genericity allows us to import in \cbv a key point of the semantics of the $\l$-calculus, namely the consistency of the \emph{smallest sensible equational theory}. Genericity indeed implies that the smallest congruence $\Hv$ (with respect to the \VSC constructors)
that: 
\begin{enumerate}
	\item contains the equational theory $=_{\vsub}$ induced by $\tovsub$, and %(that is, $=_{\vsub}$ is the symmetric, reflexive and transitive closure of $\tovsub$), and
	\item is \emph{sensible}, that is, it equates all the unsolvable terms,
\end{enumerate}
is \emph{consistent}, that is, it does not equate all terms.

\begin{theorem}
\label{thm:consistency}
$\Hv$ is consistent.
\end{theorem}

\paragraph{Axioms for Genericity and Consistency.} Kennaway et al. \cite{DBLP:journals/jflp/KennawayOV99} provide three axioms in order for an abstract notion of unsolvable term to satisfy a genericity lemma and the consistency of the theory equating all unsolvable terms. The key property behind  our direct proof, that is, the stability of $\tosolvnvar$ by substitution (\Cref{l:stability-solv-subs}), is exactly one of their axioms---the stability of unsolvable terms under substitution---just stated in  contrapositive form: \emph{if $\tm$ is unsolvable then $\tm\isub\var\tmtwo$ is unsolvable for every $\tmtwo$}.

Another of their axioms is the stability of unsolvable terms by reduction, which is an easy consequence of the normalization theorem for solving reduction.

\begin{lemma}[Stability of unsolvable terms by reduction]
Let $\tm$ be unsolvable and $\tm \tovsub \tmtwo$. Then $\tmtwo$ is unsolvable.
\end{lemma}

\begin{proof}
By contradiction. If $\tmtwo$ is solvable then by the operational characterization of  solvability, $\tosolvnvar$ terminates on $\tmtwo$, that is, $\tmtwo\tosolvnvar^{*} \solvnf$ for some solved fireball $\solvnf$. Then $\tm \tovsub^{*} \solvnf$. By the normalization property of $\tosolvnvar$ (\Cref{prop:properties-solving}.\ref{p:properties-solving-normalization-bis}), $\tosolvnvar$ terminates on $\tm$, which then is solvable---absurd.
\end{proof}

==> 99-05-Genericity.tex <==
% !TEX root = main.tex
\section{Proofs of Section \ref{sect:genericity} (Genericity)}
\ben{[lemma da adattare alla riduzione aperta]
\begin{lemma}
\label{lappendix:stability-solv-subs} % \Cref{lappendix:stability-solv-subs}.\ref{p:stability-solv-subs-one-bis}
\NoteState{l:stability-solv-subs}
\hfill
\begin{enumerate}
\item \label{p:stability-solv-subs-one-bis}
\emph{Stability of $\tosolv^{*}$ under substitution}: for all $k \geq 0$, if $\tm \tosolvnvar^{k} \tm'$ then $\tm \isub\var\tmtwo \tosolvnvar^{k} \tm'\isub\var\tmtwo$ for every $\tmtwo$.

\item \label{pappendix:stability-solv-subs-two}
\emph{Stability of solvability under removal}: if $\tm\isub\var\tmtwo$ is solvable then $\tm$ is solvable.
\end{enumerate}
\end{lemma}
}
\begin{proof}
\hfill
\begin{enumerate}
\item By a straightforward induction on $k\geq 0 $, using \Cref{l:stability-substitution}.

%%% Point 2
\item By contradiction, suppose that $\tm$ is not solvable. 
Then it is $\tosolvnvar$-divergent. By \Cref{p:stability-solv-subs-one-bis}, $\tm\isub\var\tmtwo$ is $\tosolvnvar$-divergent, and, by the operational characterization of solvability, $\tm\isub\var\tmtwo$ is unsolvable---absurd.
\qedhere
\end{enumerate}
\end{proof}



%\begin{lemma}
%\label{l:condition-solv-sequence-preserving}
%Let $\tm$ be an unsolvable term and $\tmtwo\isub\var\tm$ be a solvable term. If $\tmtwo \tosolv^{*} \tmtwo'$ then $\tmtwo \isub\var\tmthree \tosolv^{*} \tmtwo' \isub\var\tmthree$ for every term $\tmthree$.
%\end{lemma}
%
%\begin{proof}
%Let $\deriv: \tmtwo \tosolv^{*} \tmtwo'$. The proof is by induction on the number $k \defeq \sizep\deriv{\solvredsym\evarsym}$ of $\toevarsolv$ steps in $\deriv$. If $k=0$ then the statement follows by \Cref{l:stability-solv-subs}.\ref{p:stability-solv-subs-one-bis}. Otherwise, $\deriv$ has the following shape:
%\[\tmtwo \tosolvnvar^{*} \tmfour \toevarsolv\underbrace{\tmfour' \tosolv^{*} \tmtwo'}_{=\deriv'}\]
%with $\sizep{\deriv'}{\solvredsym\evarsym} = k-1$. By \Cref{l:stability-solv-subs}.\ref{p:stability-solv-subs-one-bis}, $\tmtwo\isub\var\tmthree \tosolvnvar^{*} \tmfour\isub\var\tmthree$, and by \ih $\tmfour'\isub\var\tmthree \tosolv^{*} \tmtwo'\isub\var\tmthree$. We are left to show that $\tmfour\isub\var\tmthree \toevarsolv \tmfour'\isub\var\tmthree $. We have that
%\[\tmfour = \solvctxp{\tmfour''\esub\vartwo\varthree} \toevarsolv \solvctxp{\tmfour''\isub\vartwo\varthree} = \tmfour'\]
%For some $\tmfour''$ and solving context $\solvctx$. Note that $\varthree\neq\var$ otherwise $\tmfour\isub\var\tm = \solvctx\isub\var\tm\ctxholep{\tmfour''\isub\var\tm\esub\vartwo\tm}$ would have a diverging $\tosolv$ reduction (because $\tm$ is unsolvable and $\solvctx\isub\var\tm\ctxholep{\tmfour''\isub\var\tm\esub\vartwo\ctxhole}$ is a solving context), and so would $\tmfour\isub\var\tm$, which is absurd (because it is solvable). Then 
%\[\begin{array}{lllllll}
%\tmfour\isub\var\tmthree & =&  \solvctxp{\tmfour''\esub\vartwo\varthree}\isub\var\tmthree
%\\ &= & 
%\solvctx\isub\var\tmthree\ctxholep{\tmfour''\isub\var\tmthree\esub\vartwo\varthree}
%\\ & \toevarsolv &
%\solvctx\isub\var\tmthree\ctxholep{\tmfour''\isub\var\tmthree\isub\vartwo\varthree}
%\\ & = &
%\solvctxp{\tmfour''\isub\vartwo\varthree}\isub\var\tmthree
% & = &
% \tmfour'\isub\var\tmthree
% \end{array}\]
%\end{proof}



%\begin{lemma}
%\label{l:full-norm-implies-solv-norm}
%If $\tm \tovsub^{*} \sfire$ then $\tm$ is solvable.
%\end{lemma}
%
%\begin{proof}
%	By \Cref{prop:properties-solving}.\ref{p:properties-solving-normalization}, from $\tm \tovsub^{*} \sfire$ it follows that $\tm \tosolv^{*} \tmtwo$ for some $\tosolv$-normal $\tmtwo$.
%	By \Cref{prop:operational-characterization-cbv-solv}, $\tm$ is solvable.
%\end{proof}
%\begin{proof}
%The hypothesis means that $\tm \tovsub^{*} \sfire$ with $\sfire$ full fireball. By factorization, $\tm \tosolv^{*}\tmtwo \tonsolv^{*}\sfire$ for some $\tmtwo$. Now, if in $\tmtwo$ there is a redex out of non-head abstractions, it cannot be eliminated by reducing (via $\tonsolv$) into head abstractions. Therefore, if $\tmtwo$ is not $\tosolv$-normal then $\sfire$ is not $\tosolv$-normal, absurd. Then $\tmtwo$ is $\tosolv$-normal, that is, $\tm$ is solvable.
%\end{proof}
For the proof of the genericity property we need to introduce a simple equivalence on fireballs and inert term. It states that they have the same shape out of abstractions.

\newcommand{\treq}{\sim}
\begin{definition}
Trunk equivalence $\treq$ of fireballs and inert terms is defined as follows:
\begin{itemize}
\item \emph{Inert terms}: 
\begin{itemize}
\item \emph{Variables}: $\var \treq \var$.
\item \emph{Application}: if $\itm \treq \itmtwo$ and $\fire \treq \firetwo$ then $\itm\fire \treq \itmtwo\firetwo$.
\item \emph{Substitution} if $\itm_{1} \treq \itm_{1}'$ and $\itm_{2} \treq \itm_{2}'$ then $\itm_{1}\esub\var{\itm_2} \treq \itm_{1}'\esub\var{\itm_2'}$.
\end{itemize}

\item \emph{Fireballs}: 
\begin{itemize}
\item \emph{Abstraction}: $\la\var\tm \treq \la\var\tmtwo$ for all $\tm$ and $\tmtwo$.
\item \emph{Substitution}: if $\fire \treq \firetwo$ and $\itm \treq \itmtwo$ then $\fire\esub\var\itm \treq \fire'\esub\var{\itm'}$.
\end{itemize}
\end{itemize}
\end{definition}

\begin{lemma}
\label{l:treq-properties} % \Cref{l:treq-properties}.\ref{p:treq-properties-one}
\hfill
\begin{enumerate}
\item \label{p:treq-properties-one}
\emph{Equivalence}: $\treq$ is an equivalence relation.
\item \label{p:treq-properties-two}
\emph{Stability by reduction}: if $\fire \tovsubnvar \firetwo$ then $\fire \treq\firetwo$.
\end{enumerate}
\end{lemma}

\begin{proof}
The first point is a straightforward, the second one follows from the fact that fireballs can have $\tovsubnvar$ redexes only under abstraction.
\end{proof}

\begin{lemma}[Scrutability and subterms]
\label{l:scrutable-subterms} % \reflemmap{scrutable-subterms}{ap}
\hfill
\begin{enumerate}
\item \label{p:scrutable-subterms-ap}
If $\tm\tmtwo$ is scrutable then $\tm$ and $\tmtwo$ are scrutable.

\item \label{p:scrutable-subterms-es}
If $\tm\esub\var\tmtwo$ is scrutable then $\tm$ and $\tmtwo$ are scrutable.
\end{enumerate}
\end{lemma}

\begin{proof}
It follows easily by the operational characterizations of being scrutable. Indeed if $\tm\tmtwo$ is $\tovsubo$-terminating so are $\tm$ and $\tmtwo$, and similarly for $\tm\esub\var\tmtwo$.
\end{proof}

An important point is that the previous lemma is false if one replaces \cbv inscrutable with \cbv unsolvable. In the proof, what fails is that if $\tm\esub\var\tmtwo$ is solving terminating then $\tmtwo$ might very well not be solving terminating (because solving reduction goes under abstraction), for instance $\var\esub\vartwo{\la\varthree\Omega}$ is solving terminating (because it erases $\la\varthree\Omega$ and $\tosolv$-reduces to $\var$) but $\la\varthree\Omega$ is not.

\begin{lemma}
\label{l:genericity-aux}
\hfill
\begin{enumerate}
\item If $\tm$ is inscrutable and $\itm\isub\var\tm$ is scrutable then $\itm\isub\var\tm \treq \itm$.
\item If $\tm$ is inscrutable and $\fire\isub\var\tm$ is scrutable then  $\fire\isub\var\tm \treq \fire$.
\end{enumerate}
\end{lemma}

\begin{proof}
The two points are proved together by mutual induction on $\itm$ and $\fire$.
\begin{enumerate}
\item Cases of $\itm$:
\begin{itemize}
\item \emph{Variable}, that is, $\itm = \vartwo$. Then $\vartwo\neq\var$ otherwise $\itm\isub\var\tm = \tm$ would be inscrutable. Then $\itm\isub\var\tm = \vartwo\isub\var\tm = \vartwo \treq \vartwo = \itm$.

\item \emph{Application}, that is, $\itm = \itmtwo \fire$. Then $\itm\isub\var\tm = \itmtwo\isub\var\tm \fire\isub\var\tm$. By \reflemmap{scrutable-subterms}{ap}, both $\itmtwo\isub\var\tm$ and $\fire\isub\var\tm$ are scrutable, and so we can apply the \ih and obtain $\itmtwo\isub\var\tm \fire\isub\var\tm \treq_{\ih 1} \itmtwo \fire\isub\var\tm \treq_{\ih 2} \itmtwo \fire = \itm$.

\item \emph{Substitution}, that is, $\itm = \itm_{1}\esub\vartwo{\itm_{2}}$. Then $\itm\isub\var\tm = \itm_{1}\isub\var\tm \esub\vartwo{\itm_{2}\isub\var\tm}$. By \reflemmap{scrutable-subterms}{es}, both $\itm_{1}\isub\var\tm$ and $\itm_{2}\isub\var\tm$ are scrutable, and so we can apply the \ih and obtain  $\itm_{1}\isub\var\tm \esub\vartwo{\itm_{2}\isub\var\tm}\treq_{\ih 1} \itm_{1} \esub\vartwo{\itm_{2}} = \itm$.
\end{itemize}

\item Cases of $\fire$:
\begin{itemize}
\item \emph{Abstraction}, that is, $\fire = \la\vartwo\tmtwo$. Then $\fire\isub\var\tm = \la\vartwo(\tmtwo\isub\var\tm) \treq \la\vartwo\tmtwo = \fire$.

\item \emph{inert}, that is, $\fire = \itm$. Then $\fire\isub\var\tm = \itm\isub\var\tm \treq_{\ih 1} \itm$.

\item \emph{Substitution}, that is, $\fire = \firetwo\esub\vartwo{\itm}$. Then $\fire\isub\var\tm = \firetwo\isub\var\tm \esub\vartwo{\itm\isub\var\tm}$. By \reflemmap{scrutable-subterms}{es}, both $\firetwo\isub\var\tm$ and $\itm\isub\var\tm$ are scrutable, and so we can apply the \ih and obtain $\firetwo\isub\var\tm \esub\vartwo{\itm\isub\var\tm} \treq_{\ih 1} \firetwo\isub\var\tm \esub\vartwo{\itm} \treq_{\ih 2} \fire\esub\vartwo{\itm} = \fire.$
\end{itemize}

\end{enumerate}
\end{proof}

\begin{theorem}[Genericity of inscrutable terms]
	\label{thmappendix:genericity}
	\NoteState{thm:genericity}
Let $\tm$ be an inscrutable term and $\tmtwo$ be a full normal form.
\begin{enumerate}
\item \label{pappendix:genericity-as-subs}
\emph{Genericity as substitution}:
if $\tmthree \isub\var\tm \tovsub^{*} \tmtwo$ then $\tmthree \isub\var\tmfour \tovsub^{*} \tmtwo$ for every term $\tmfour$.

\item \emph{Genericity as context}:
if $\ctxp\tm \tovsub^{*} \tmtwo$ then $\ctxp\tmthree \tovsub^{*} \tmtwo$ for every term $\tmthree$.
\end{enumerate}
\end{theorem}


\begin{proof}
\hfill
\begin{enumerate}
\item We rather prove the following statement where $\tmtwo$ is replaced by a full fireball $\sfire$:
\begin{center}
Let $\tm$ be an inscrutable term and $\sfire$ a full fireball. If $\tmtwo \isub\var\tm \tovsubnvar^{*} \sfire$ then $\tmtwo \isub\var\tmthree \tovsubnvar^{*} \sfire$ for every term $\tmthree$.
\end{center}
By irrelevance of $\toevar$ (\Cref{prop:irrelevance}), the new statement is equivalent to the original one. Indeed, if $\tmthree \isub\var\tm \tovsub^{*} \tmtwo$ with $\tmtwo$ full normal then $\tovsubnvar$ normalizes, that is, $\tmtwo \isub\var\tm \tovsubnvar^{*} \sfire$ with $\sfire \tovsub^{*} \tmtwo$ by confluence. By the new statement, $\tmtwo \isub\var\tmthree \tovsubnvar^{*} \sfire$, and so $\tmtwo \isub\var\tmthree \tovsub^{*} \tmtwo$.\medskip

The proof of the new statement is by induction on $\sfire$. 
%If $\tmtwo \isub\var\tm \tovsubnvar^{*} \sfire$ then, by irrelevance of $\toevarsolv$, $\tmtwo \isub\var\tm \tovsub^{*} \sfire'$ with $\sfire'$ full normal. 
By the normalization property of $\tovsubonvar$ (\Cref{prop:properties-open-extra}.\ref{p:properties-open-extra-normalization-bis}), $\tmtwo  \tovsubonvar^{*} \fire $ for some fireball $\fire$.
By stability of reduction under substitutions (\Cref{lappendix:stability-solv-subs}.\ref{p:stability-solv-subs-one-bis}),
 we have both 
$\tmtwo \isub\var\tm \tovsubonvar^{*} \fire \isub\var\tm$ and $\tmtwo \isub\var\tmthree \tovsubonvar^{*} \fire\isub\var\tmthree$. By confluence, $\fire \isub\var\tm \tovsubnvar^{*} \sfire$. We are left to prove that $\fire\isub\var\tmthree  \tovsubnvar^{*}\sfire$. Cases of $\fire$:
\begin{enumerate}
\item \emph{Abstraction}, that is, $\fire = \la\vartwo\tmfour$. Then 
\[\fire\isub\var\tm = \la\vartwo\tmfour\isub\var\tm \tovsubnvar^{*}\sfire = \la\vartwo\sfiretwo\]
with $\tmfour\isub\var\tm \tovsubnvar^{*}\sfiretwo$ for some $\sfiretwo$. By \ih, $\tmfour\isub\var\tmthree \tovsubnvar^{*}\sfiretwo$ for all $\tmthree$, and so 
\[\fire\isub\var\tmthree = \la\vartwo\tmfour\isub\var\tmthree  \tovsubnvar^{*}\la\vartwo\sfiretwo = \sfire.\] 

\item \emph{Inert}, that is, $\fire = \itm$. Three sub-cases:
\begin{itemize}
\item \emph{Variable}, that is, $\fire = \vartwo$. Note that $\vartwo \neq \var$, otherwise $\fire\isub\var\tm = \var\isub\var\tm = \tm$ would be inscrutable and so $\tovsubnvar$ divergent, contradicting $\fire \isub\var\tm \tovsubnvar^{*} \sfire$. Then $\fire\isub\var\tm = \vartwo\isub\var\tm = \vartwo = \sfire$, and similarly $\fire\isub\var\tmthree = \vartwo\isub\var\tmthree = \vartwo = \sfire$. 

\item \emph{Application}, that is, $\fire = \itm \firetwo$. By \Cref{l:genericity-aux}, $\fire\treq \fire\isub\var\tm$, that is, $\fire\isub\var\tm = \itm\isub\var\tm \firetwo\isub\var\tm = \itmtwo \firethree$ for some $\itmtwo$ and $\firethree$. Then:
\[\fire\isub\var\tm = \itm\isub\var\tm \firetwo\isub\var\tm = \itmtwo \firethree \tovsubnvar^{*}\sfire =_{L.\ref{l:treq-properties}.\ref{p:treq-properties-two}} \itmthree \firefour\]
with $\itm\isub\var\tm \tovsubnvar^{*} \itmthree$ and $\firetwo\isub\var\tm \tovsubnvar^{*} \firefour$. Note that $\itmthree$ and  $\firefour$ actually are full fireballs because they are sub-terms of $\sfire$. Then we can apply the \ih, obtaining $\itm\isub\var\tmthree \tovsubnvar^{*} \itmthree$ and $\firetwo\isub\var\tmthree \tovsubnvar^{*} \firefour$ for all $\tmthree$, so that:
\[\fire\isub\var\tmthree  =\itm\isub\var\tmthree \firetwo\isub\var\tmthree \tovsubnvar^{*} \itmthree\firefour= \sfire.\] 

\item \emph{Substitution}, that is, $\fire = \itm_1 \esub\vartwo{\itm_2}$. By \Cref{l:genericity-aux}, $\fire\treq \fire\isub\var\tm$, that is, $\fire\isub\var\tm = \itm_1\isub\var\tm \esub\vartwo{\itm_2\isub\var\tm} = \itm_1' \esub\vartwo{\itm_2'}$ for some $\itm_{1}'$ and $\itm_{2}'$. Then:
\[\fire\isub\var\tm = \itm_1\isub\var\tm \esub\vartwo{\itm_2\isub\var\tm} = \itm_1' \esub\vartwo{\itm_2'} \tovsubnvar^{*}\sfire =_{L.\ref{l:treq-properties}.\ref{p:treq-properties-two}} \itm_1'' \esub\vartwo{\itm_2''}\]
with $\itm_{1}\isub\var\tm \tovsubnvar^{*} \itm_{1}''$ and $\itm_{2}\isub\var\tm \tovsubnvar^{*} \itm_{2}''$.  Note that $\itm_1''$ and  $\itm_2''$ actually are full fireballs because they are sub-terms of $\sfire$. Then we can apply the \ih, obtaining $\itm_{1}\isub\var\tmthree \tovsubnvar^{*} \itm_{1}''$ and $\itm_{2}\isub\var\tmthree \tovsubnvar^{*} \itm_{2}''$ for all $\tmthree$, so that 
\[\fire\isub\var\tmthree = \itm_{1}\isub\var\tmthree\esub\vartwo{\itm_{2}\isub\var\tmthree} \tovsubnvar^{*}\itm_{1}'' \esub\vartwo{\itm_{2}''} = \sfire.\] 
\end{itemize}

\item \emph{Fireball with inert substitution}, that is, $\fire =  \firetwo\esub\vartwo{\itm}$. By \Cref{l:genericity-aux}, $\fire\treq \fire\isub\var\tm$, that is, $\fire\isub\var\tm = \firetwo\isub\var\tm \esub\vartwo{\itm\isub\var\tm}= \firethree\esub\vartwo\itmtwo$ for some $\firethree$ and $\itmtwo$. Then:
\[\fire\isub\var\tm = \firetwo\isub\var\tm\esub\vartwo{\itm\isub\var\tm} = \firethree\esub\vartwo\itmtwo \tovsubnvar^{*}\sfire =_{L.\ref{l:treq-properties}.\ref{p:treq-properties-two}} \firefour\esub\vartwo{\itmthree}\]
with $\firetwo\isub\var\tm \tovsubnvar^{*} \firefour$ and $\itm\isub\var\tm \tovsubnvar^{*} \itmthree$. 
Note that $\firefour$ and  $\itmthree$ actually are full fireballs because they are sub-terms of $\sfire$. Then we can apply the \ih, obtaining 
$\firetwo\isub\var\tmthree \tovsubnvar^{*} \firefour$ and $\itm\isub\var\tmthree \tovsubnvar^{*}\itmthree$ for all $\tmthree$, so that
\[\fire\isub\var\tmthree =\firetwo\isub\var\tmthree\esub\vartwo{\itm\isub\var\tmthree} \tovsubnvar^{*} \firefour \esub\vartwo\itmthree = \sfire.\] 
\end{enumerate}

% POINT 2
\item
Let $\fv\tm \cup \fv\tmthree = \set{\var_{1},\ldots,\var_{k}}$, and $\vartwo$ be a variable fresh with respect to $\fv\tm \cup \fv\tmthree\cup\fv\ctx$ and not captured by $\ctx$. Consider $\tmfour \defeq \ctxp{\vartwo \var_{1} \ldots \var_{k}}$, and note that:
\[\begin{array}{llllll}
\tmfour\isub\vartwo{\la{\var_{1}}\ldots\la{\var_{k}}\tm} = \ctxp{(\la{\var_{1}}\ldots\la{\var_{k}}\tm) \var_{1} \ldots \var_{k}} \tovsub^{2k} \ctxp\tm
\end{array}\]
The fact that $\tm$ is unsolvable implies that $\la{\var_{1}}\ldots\la{\var_{k}}\tm$ is also unsolvable. Since 
\[\tmfour\isub\vartwo{\la{\var_{1}}\ldots\la{\var_{k}}\tm} \tovsub^{*}\ctxp\tm \tovsub^{*}\tmtwo\]
 we are in the hypotheses of \Cref{thm:genericity}.\ref{p:genericity-as-subs}. 
 By that lemma, $\tmfour\isub\vartwo{\tmthree'} \tovsub^{*}\tmtwo$ for all $\tmthree'$. In particular, take $\tmthree' = \la{\var_{1}}\ldots\la{\var_{k}}\tmthree$, and note that 
\[\tmfour\isub\vartwo{\la{\var_{1}}\ldots\la{\var_{k}}\tmthree} \tovsub^{*}\ctxp\tmthree\]
By confluence, $\ctxp\tmthree \tovsub^{*} \tmtwo$.
\qedhere
\end{enumerate}
 \end{proof}
